AURORA: Autonomous Updating of ROM and Controller via Recursive Adaptation

Real time model based control of high dimensional nonlinear systems presents severe computational challenges. Conventional reduced order model control relies heavily on expert tuning or parameter adaptation and seldom offers mechanisms for online supervised reconstruction. We introduce AURORA, Autonomous Updating of ROM and Controller via Recursive Adaptation, a supervisory framework that automates ROM based controller design and augments it with diagnostic triggered structural adaptation. Five specialized agents collaborate through iterative generate judge revise cycles, while an Evaluation Agent classifies performance degradation into three operationally distinct categories, subspace inadequacy, parametric drift, and control inadequacy, and routes corrective action to the responsible agent. For linear ROMs, we analytically prove that this classification is correct under mild assumptions and that the supervisory switching cycle preserves exponential stability subject to a dwell time condition. For nonlinear systems, the absence of a universal Lyapunov construction for autonomously discovered ROM structures precludes analogous analytical guarantees, so we validate the same classification empirically. Experiments on eight benchmark systems with state dimensions up to 5177 compare AURORA against expert tuned baselines, gain scheduled control, and online RLS adaptive alternatives. Controlled fault injection experiments confirm 91 percent diagnostic routing accuracy. AURORA achieves 6 to 12 percent tracking improvement over expert baselines and 4 to 5 percent over classical adaptive alternatives.

==> newbib.tex <==
@book{rawlings2017model,
  title={Model Predictive Control: Theory, Computation, and Design},
  author={Rawlings, James B and Mayne, David Q and Diehl, Moritz},
  year={2017},
  edition={2nd},
  publisher={Nob Hill Publishing}
}

@book{isidori1995nonlinear,
  title={Nonlinear Control Systems: an introduction},
  author={Isidori, Alberto},
  year={1985},
  publisher={Springer-Verlag}
}

@book{kirk2004optimal,
  title={Optimal Control Theory: An Introduction},
  author={Kirk, Donald E},
  year={2004},
  publisher={Dover Publications}
}

@article{benner2015survey,
  title={A survey of projection-based model reduction methods for parametric dynamical systems},
  author={Benner, Peter and Gugercin, Serkan and Willcox, Karen},
  journal={SIAM Review},
  volume={57},
  number={4},
  pages={483--531},
  year={2015},
  publisher={SIAM}
}

@book{brunton2019data,
  title={Data-Driven Science and Engineering: Machine Learning, Dynamical Systems, and Control},
  author={Brunton, Steven L and Kutz, J Nathan},
  year={2019},
  publisher={Cambridge University Press}
}

@book{holmes2012turbulence,
  title={Turbulence, Coherent Structures, Dynamical Systems and Symmetry},
  author={Holmes, Philip},
  year={2012},
  edition={2nd},
  publisher={Cambridge University Press}
}

@article{sirovich1987turbulence,
  title={Turbulence and the dynamics of coherent structures. {Part I}: Coherent structures},
  author={Sirovich, Lawrence},
  journal={Quarterly of Applied Mathematics},
  volume={45},
  number={3},
  pages={561--571},
  year={1987}
}

@article{chaturantabut2010nonlinear,
  title={Nonlinear model reduction via discrete empirical interpolation},
  author={Chaturantabut, Saifon and Sorensen, Danny C},
  journal={SIAM Journal on Scientific Computing},
  volume={32},
  number={5},
  pages={2737--2764},
  year={2010},
  publisher={SIAM}
}

@article{mayne2000constrained,
  title={Constrained model predictive control: Stability and optimality},
  author={Mayne, David Q and Rawlings, James B and Rao, Christopher V and Scokaert, Pierre OM},
  journal={Automatica},
  volume={36},
  number={6},
  pages={789--814},
  year={2000},
  publisher={Elsevier}
}

@article{halko2011finding,
  title={Finding structure with randomness: Probabilistic algorithms for constructing approximate matrix decompositions},
  author={Halko, Nathan and Martinsson, Per-Gunnar and Tropp, Joel A},
  journal={SIAM Review},
  volume={53},
  number={2},
  pages={217--288},
  year={2011},
  publisher={SIAM}
}

@article{wei2022chain,
  title={Chain-of-thought prompting elicits reasoning in large language models},
  author={Wei, Jason and Wang, Xuezhi and Schuurmans, Dale and Bosma, Maarten and Xia, Fei and Chi, Ed and Le, Quoc V and Zhou, Denny},
  journal={Advances in Neural Information Processing Systems},
  volume={35},
  pages={24824--24837},
  year={2022}
}

@book{narendra1989stable,
  title        = {Stable Adaptive Systems},
  author       = {Narendra, Kumpati S. and Annaswamy, Anuradha M.},
  year         = {2012},
  publisher    = {Courier Corporation}
}

@book{astrom2013adaptive,
  title={Adaptive Control},
  author={{\AA}str{\"o}m, Karl Johan and Wittenmark, Bj{\"o}rn},
  year={2008},
  edition={2nd},
  publisher={Dover Publications}
}

@article{li2025generative,
  title        = {Generative AI and CAD Automation for Diverse and Novel Mechanical Component Designs under Data Constraints},
  author       = {Li, Kun-Ying and Huang, Cheng-Kai and Chen, Qing-Wei and Zhang, Hsuan-Cheng and Tang, Tsann-Tay},
  journal      = {Discover Applied Sciences},
  volume       = {7},
  number       = {4},
  pages        = {1--21},
  year         = {2025},
  publisher    = {Springer Nature},
  doi          = {10.1007/s44247-025-00184-9}
}

@article{zhang2025large,
  title        = {Large Language Models for Computer-Aided Design: A Survey},
  author       = {Zhang, Licheng and Le, Bach and Akhtar, Naveed and Lam, Siew-Kei and Ngo, Tuan},
  journal      = {arXiv preprint arXiv:2505.08137},
  year         = {2025},
}

@article{wang2024survey,
  title={A survey on large language model based autonomous agents},
  author={Wang, Lei and Ma, Chen and Feng, Xueyang and Zhang, Zeyu and Yang, Hao and Zhang, Jingsen and Chen, Zhiyuan and Tang, Jiakai and Chen, Xu and Lin, Yankai and others},
  journal={Frontiers of Computer Science},
  volume={18},
  number={6},
  pages={186345},
  year={2024},
  publisher={Springer}
}

@article{wu2023autogen,
  title={{AutoGen}: Enabling next-generation {LLM} applications via multi-agent conversation},
  author={Wu, Qingyun and Bansal, Gagan and Zhang, Jieyu and Wu, Yiran and Li, Beibin and Zhu, Erkang and Jiang, Li and Zhang, Xiaoyun and Zhang, Shaokun and Liu, Jiale and others},
  journal={arXiv preprint arXiv:2308.08155},
  year={2023}
}

@article{shinn2023reflexion,
  title={Reflexion: Language agents with verbal reinforcement learning},
  author={Shinn, Noah and Cassano, Federico and Gopinath, Ashwin and Narasimhan, Karthik and Yao, Shunyu},
  journal={Advances in Neural Information Processing Systems},
  volume={36},
  pages={8634--8652},
  year={2023}
}

@article{madaan2024self,
  title={Self-refine: Iterative refinement with self-feedback},
  author={Madaan, Aman and Tandon, Niket and Gupta, Prakhar and Hallinan, Skyler and Gao, Luyu and Wiegreffe, Sarah and Alon, Uri and Dziri, Nouha and Prabhumoye, Shrimai and Yang, Yiming and others},
  journal={Advances in Neural Information Processing Systems},
  volume={36},
  pages={46534--46594},
  year={2023}
}

@article{guo2024controlagent,
  title={{ControlAgent}: Automating control system design via novel integration of {LLM} agents and domain expertise},
  author={Guo, Xingang and Keivan, Darioush and Syed, Usman and Qin, Lianhui and Zhang, Huan and Dullerud, Geir and Seiler, Peter and Hu, Bin},
  journal={arXiv preprint arXiv:2410.19811},
  year={2024}
}

@article{liang2024lmpc,
  title={Learning to learn faster from human feedback with language model predictive control},
  author={Liang, Jacky and Xia, Fei and Yu, Wenhao and Zeng, Andy and Arenas, Montse Gonzalez and Attarian, Maria and Bauza, Maria and Bennice, Matthew and Bewley, Alex and Dostmohamed, Adil and others},
  journal={arXiv preprint arXiv:2402.11450},
  year={2024}
}

@article{hafez2025safe,
  title={Safe {LLM}-controlled robots with formal guarantees via reachability analysis},
  author={Hafez, Ahmed and Akhormeh, Amin Nikanjam and Hegazy, Ahmed and Alanwar, Amr},
  journal={arXiv preprint arXiv:2503.03911},
  year={2025}
}

@article{lorenzen2017adaptive,
  title        = {Adaptive Model Predictive Control with Robust Constraint Satisfaction},
  author       = {Lorenzen, Matthias and Allg{\"o}wer, Frank and Cannon, Mark},
  journal      = {IFAC-PapersOnLine},
  volume       = {50},
  number       = {1},
  pages        = {3313--3318},
  year         = {2017},
  publisher    = {Elsevier},
  doi          = {10.1016/j.ifacol.2017.08.551}
}

@article{ahmed2024adversarially,
  title        = {Adversarially Robust Reduced Order Model Predictive Control: Balancing Performance and Efficiency},
  author       = {Ahmed, Akhil and del Rio-Chanona, Ehecatl Antonio and Mercang{\"o}z, Mehmet},
  journal      = {IFAC-PapersOnLine},
  volume       = {58},
  number       = {28},
  pages        = {378--383},
  year         = {2024},
  publisher    = {Elsevier},
  doi          = {10.1016/j.ifacol.2024.12.173}
}

@inproceedings{buerger2024safe,
  title        = {Safe Learning in Nonlinear Model Predictive Control},
  author       = {Buerger, Johannes and Cannon, Mark and Doff-Sotta, Martin},
  booktitle    = {6th Annual Learning for Dynamics \& Control Conference},
  pages        = {603--614},
  year         = {2024},
  organization = {PMLR},
  month        = jun,
  series       = {Proceedings of Machine Learning Research},
}

@article{muller2016economic,
  title        = {Economic Model Predictive Control without Terminal Constraints for Optimal Periodic Behavior},
  author       = {M{\"u}ller, Matthias A. and Gr{\"u}ne, Lars},
  journal      = {Automatica},
  volume       = {70},
  pages        = {128--139},
  year         = {2016},
  publisher    = {Elsevier},
  doi          = {10.1016/j.automatica.2016.03.024}
}

@article{brunton2016discovering,
  title={Discovering governing equations from data by sparse identification of nonlinear dynamical systems},
  author={Brunton, Steven L and Proctor, Joshua L and Kutz, J Nathan},
  journal={Proceedings of the National Academy of Sciences},
  volume={113},
  number={15},
  pages={3932--3937},
  year={2016},
  publisher={National Acad Sciences}
}

@incollection{chahlaoui2005benchmark,
  title={Benchmark Examples for Model Reduction of Linear Time-Invariant Dynamical Systems},
  author={Chahlaoui, Younes and Van Dooren, Paul},
  booktitle={Dimension Reduction of Large-Scale Systems},
  editor={Benner, Peter and Sorensen, Danny C and Mehrmann, Volker},
  series={Lecture Notes in Computational Science and Engineering},
  volume={45},
  pages={379--392},
  year={2005},
  publisher={Springer},
  address={Berlin, Heidelberg}
}

@article{carlberg2015galerkin,
  title={Galerkin v. least-squares {Petrov-Galerkin} projection in nonlinear model reduction},
  author={Carlberg, Kevin and Bou-Mosleh, Charbel and Farhat, Charbel},
  journal={Journal of Computational Physics},
  volume={330},
  pages={693--734},
  year={2015},
  publisher={Elsevier}
}

@inproceedings{hong2023metagpt,
  title        = {{MetaGPT}: Meta Programming for a Multi-Agent Collaborative Framework},
  author       = {Hong, Sirui and Zhuge, Mingchen and Chen, Jonathan and Zheng, Xiawu and Cheng, Yuheng and Wang, Jinlin and Zhang, Ceyao and Wang, Zihan and Yau, Siew-Kei S. and Lin, Zhen and Zhou, Lian and Schmidhuber, Jürgen},
  booktitle    = {The Twelfth International Conference on Learning Representations},
  year         = {2024},
  organization = {ICLR},
}

